Enabling Real-Time Programmability for RAN Functions: A Wasm-Based Approach for Isolated and Deterministic dApps

The Open Radio Access Network Alliance (O-RAN) architecture enables third-party applications to optimize Radio Access Networks (RANs) at multiple timescales. However, the real-time distributed applications (known as dApps) that demand low latency, high performance, and resource isolation remain underexplored. Existing approaches propose collocating a new RAN Intelligent Controller (RIC) at the edge, or deploying dApps in bare metal along with RAN functions. The former approach increases network complexity and requires additional edge computing resources, and the latter raises serious security concerns due to the lack of native mechanisms to isolate dApps and RAN functions. Meanwhile, WebAssembly (Wasm) has emerged as a fast, lightweight technology for robust execution of external, untrusted code. In this work, we propose a new approach to executing dApps using Wasm to isolate applications in real-time in O-RAN. Results from a proof-of-concept implementation show that our lightweight and robust approach can provide predictable, deterministic performance, resource isolation, and low latency, supporting real-time control loops.

==> acronyms.tex <==
\DeclareAcronym{RAN}{
    short = {RAN},
    long  = {Radio Access Network},
}

\DeclareAcronym{O-RAN}{
    short = {O-RAN},
    long  = {Open Radio Access Network Alliance},
}

\DeclareAcronym{RIC}{
    short = {RIC},
    long  = {RAN Intelligent Controller},
}

\DeclareAcronym{RLC}{
    short = {RLC},
    long  = {Radio Link Control},
}

\DeclareAcronym{FPGA}{
    short = {FPGA},
    long  = {Field-Programmable Gate Array},
}

\DeclareAcronym{GPU}{
    short = {GPU},
    long  = {Graphics Processing Unit},
}

\DeclareAcronym{DPU}{
    short = {DPU},
    long  = {Data Processing Unit},
}

\DeclareAcronym{QoS}{
    short = {QoS},
    long  = {Quality of Service},
}

\DeclareAcronym{AOT}{
    short = {AOT},
    long  = {Ahead-Of-Time},
}

\DeclareAcronym{DPDK}{
    short = {DPDK},
    long  = {Data Plane Development Kit},
}

\DeclareAcronym{eBPF}{
    short = {eBPF},
    long  = {extended Berkeley Packet Filter},
}

\DeclareAcronym{XDP}{
    short = {XDP},
    long  = {eXpress Data Path},
}

\DeclareAcronym{SMO}{
    short = {SMO},
    long  = {Service Management and Orchestration},
}


\DeclareAcronym{PRB}{
    short = {PRB},
    long  = {Physical Resource Block},
}

\DeclareAcronym{OAI}{
    short = {OAI},
    long  = {OpenAir Interface},
}

\DeclareAcronym{Near-RT RIC}{
    short = {Near-RT RIC},
    long  = {Near Real-Time \ac{RIC}},
}

\DeclareAcronym{Non-RT RIC}{
    short = {Non-RT RIC},
    long  = {Non Real-Time \ac{RIC}},
}

\DeclareAcronym{RT-RIC}{
    short = {RT-RIC},
    long  = {Real-Time \ac{RIC}},
}

\DeclareAcronym{RU}{
    short = {RU},
    long  = {Radio Unit},
}

\DeclareAcronym{DU}{
    short = {DU},
    long  = {Distributed Unit},
}

\DeclareAcronym{CU}{
    short = {CU},
    long  = {Central Unit},
}

\DeclareAcronym{MNO}{
    short = {MNO},
    long  = {Mobile Network Operator},
}

\DeclareAcronym{AI}{
    short = {AI},
    long  = {Artificial Intelligence},
}

\DeclareAcronym{ML}{
    short = {ML},
    long  = {Machine Learning},
}

\DeclareAcronym{KPI}{
    short = {KPI},
    long  = {Key Performance Indicator},
}

\DeclareAcronym{Wasm}{
    short = {Wasm},
    long  = {WebAssembly},
}

\DeclareAcronym{BS}{
    short = {BS},
    long  = {Base Station},
}

\DeclareAcronym{TTI}{
    short = {TTI},
    long  = {Transmission Time Interval},
}

\DeclareAcronym{SC}{
    short = {SC},
    long  = {Software Community},
}

\DeclareAcronym{AoT}{
    short = {AoT},
    long  = {Ahead-of-time},
}

\DeclareAcronym{JIT}{
    short = {JIT},
    long  = {Just-in-time},
}

\DeclareAcronym{SIMD}{
    short = {SIMD},
    long  = {Single Instruction, Multiple Data},
}

\DeclareAcronym{RF}{
    short = {RF},
    long  = {Radio Frequency},
}
